MonoGS++: Fast and Accurate Monocular RGB Gaussian SLAM

We present MonoGS++, a novel fast and accurate Simultaneous Localization and Mapping (SLAM) method that leverages 3D Gaussian representations and operates solely on RGB inputs. While previous 3D Gaussian Splatting (GS)-based methods largely depended on depth sensors, our approach reduces the hardware dependency and only requires RGB input, leveraging online visual odometry (VO) to generate sparse point clouds in real-time. To reduce redundancy and enhance the quality of 3D scene reconstruction, we implemented a series of methodological enhancements in 3D Gaussian mapping. Firstly, we introduced dynamic 3D Gaussian insertion to avoid adding redundant Gaussians in previously well-reconstructed areas. Secondly, we introduced clarity-enhancing Gaussian densification module and planar regularization to handle texture-less areas and flat surfaces better. We achieved precise camera tracking results both on the synthetic Replica and real-world TUM-RGBD datasets, comparable to those of the state-of-the-art. Additionally, our method realized a significant 5.57x improvement in frames per second (fps) over the previous state-of-the-art, MonoGS.

==> figures/add.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.4\textwidth]{assets/add.png}
    \caption{\textbf{Add new 3D Gaussians.} The newly coming point clouds will be estimated their positional redundancy before seeding a new 3D Gaussian.}
    % For the newly coming frame $I_j$ along with its optimized pose $T_j$, the back-projected point will seed a new 3D Gaussian if the distance is not too close to the means of well reconstructed existing Gaussians, otherwise the point is dropped off.
    \label{fig:fig_add}
\end{figure*}

==> figures/supp_clarity.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.95\textwidth]{assets/supp_clarity.png}
    \caption{Visual comparison results of with and without Clarity-Enhancing Densification.}
    \label{fig:fig_supp_clarity}
\end{figure*}

==> figures/supp_plane.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.85\textwidth]{assets/supp_plane.png}
    \caption{Loss curve of our method with and without planar regularization.}
    \label{fig:fig_supp_plane}
\end{figure*}

==> figures/supp_vis1.tex <==
\begin{figure*}[htbp]
    \centering
    \includegraphics[width=0.95\textwidth]{assets/supp_fig1.png}
    \caption{Rendering samples on Replica dataset.}
    \label{fig:fig_supp_fig1}
\end{figure*}

==> figures/supp_vis2.tex <==
\begin{figure*}[htbp]
    \centering
    \includegraphics[width=0.95\textwidth]{assets/supp_fig2.png}
    \caption{Rendering samples on Replica dataset.}
    \label{fig:fig_supp_fig2}
\end{figure*}

==> internal_review.tex <==
R: review from Zhou Dong
Besides the promising exp results, not fully understand the contributions here:
seems like just use 3D-GS could increase FPS. Maybe some nerf-based work like SMERF is comparable with 3DGS in their work. Should we explain more details or ablation study to prove our method?
How could your framework handle RGB-D&RGB, is there any special design between ours and others (only on RGB)? Or do we have some explanation here to make readers more clear.
I know it's a draft version, but looks like a little bit confused to get the points of this paper.
A: 
1. current nerf-based or gaussian-based slam need jointly optimize the tracking and mapping process, although it seems reasonable under the online setting in SLAM application, I argue that the iterative optimization is expensive and not accurate enough for tracking, existing lightweight visual odometry is enough to provide accurate camera poses, the heavy optimization (with respect to the compute consuming nerf and gaussians)  seems unnecessary. That's why our system employ DPVO is far faster than others also use 3D-GS while achieving the lowest tracking error.
2. how to initialize or seed 3D Gaussians in online SLAM system is a critical question. current Gaussian based slams choose to directly use available depth map to initialize point cloud (where gaussians are then created), which contrains their application with monocular camera without depth sensor. In comparison, under RGB setting, we only need the depths estimated from DepthAnything in the initial stage (8 keyframes only, short time period), then during tracking, DPVO will update depths of patches, we can discard the usage of DepthAnything afterwards, the patches can be used to seed new points (Gaussians). In the RGB-D mode, it's trivial to replace the estimated depth by the depths from input depth maps.
3. I have not read SMERF, it can be treated as a basline if we replace the implicit representation by it in existing nerf-based slam systems. But I think it is to some extent beyond our work.
4. ablation studies and other novelty improvements (e.g., loop detection, re-localization) will be added in the next one to two weeks.

----------------------------------------------------------------------------------

R: review from Ji Liu
1. 第一节的 motivation 不是很清楚，为什么，解决什么问题
A: please see answer 1/2 to Zhou Dong
2. 第二节末尾可以讨论一下和相似方法的区别
A: related works? have discussed in Introduction.
3. 第三节 开始部分需要整体介绍一下方法和重要部分，有个整体的 overview
A: Yes, done.
4. 方法部分写的太简单，不是很具体，文章的是否具有创新，还是的简单sota 相加？
方法部分会加上图和更多解释，帮助读者理解
A: other novelty improvements (e.g., loop detection, re-localization) will be added in the next one to two weeks.

==> tables/supp_memory.tex <==
\begin{table}[htbp]
    \centering
    \resizebox{0.65\textwidth}{!}{
    \begin{tabular}{cccc}
    \hline
      Method          &  SplaTAM~\cite{splatam} & MonoGS~\cite{monogs} & Ours \\ \hline
      GPU Memory (MB)    &  11611 & 15315 & 8104 \\ \hline    
    \end{tabular}
    }
    \caption{\textbf{GPU memory consumption comparison.} We compare GPU memory consumption with baselines SplaTAM~\cite{splatam} and MonoGS~\cite{monogs} on Replica/room0.}
    \label{tab:tab:memory}
\end{table}

==> tables/supp_rgbd.tex <==
\begin{table}[htbp]
\centering
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{ccccccccc}
\hline
Method        & Modality & Metric                   & room2 & office2 & office4 & fr1/desk2                     & fr2/xyz                       & fr3/office                     \\ \hline
MonoGS        & RGB      & PSNR{[}dB{]}$\uparrow$   & 31.82 & 27.01   & 27.29   & 14.06                         & 22.06                         & 23.02 \\
              &          & SSIM$\uparrow$           & 0.92  & 0.88    & 0.90    & 0.50                          & 0.72                          & 0.78                           \\
              &          & LPIPS$\downarrow$        & 0.16  & 0.26    & 0.25    & 0.62                          & 0.27                          & 0.32                           \\
              &          & ATE-MSE (cm)$\downarrow$ & 6.53  & 20.89   & 43.85   & 79.45                         & 4.31                          & 1.85  \\ \hline
MonoGS        & RGB-D    & PSNR{[}dB{]}$\uparrow$   & \underline{37.49} & \underline{36.24}   & 37.06   & 8.90                          & 12.46                         & 15.95                          \\
              &          & SSIM$\uparrow$           & \underline{0.96}  & \textbf{0.96}    & \underline{0.95}    & 0.31                          & 0.71                          & 0.46                           \\
              &          & LPIPS$\downarrow$        & 0.075 & \textbf{0.078}   & 0.099   & 0.71                          & 0.30                          & 0.74                           \\
              &          & ATE-MSE (cm)$\downarrow$ & 0.31  & \textbf{0.31}    & 3.2     & 90.92                         & 1.47                          & 104.88                         \\ \hline
\textbf{Ours} & RGB      & PSNR{[}dB{]}$\uparrow$   & 37.01 & 36.11   & 37.28   & \underline{20.64}                & \underline{26.52}                & \underline{25.08}                 \\
              &          & SSIM$\uparrow$           & \underline{0.96}  & \underline{0.95}    & \textbf{0.96}    & \underline{0.77} & \underline{0.86} & \underline{0.85}                  \\
              &          & LPIPS$\downarrow$        & \underline{0.077} & 0.090   & \underline{0.086}   & \underline{0.29}                 & \underline{0.13}                 & \underline{0.18}                  \\
              &          & ATE-MSE (cm)$\downarrow$ & \underline{0.22}  & 0.42    & \underline{0.42}    & \underline{5.18}                          & \textbf{0.38}                 & \underline{0.36}                  \\ \hline
\textbf{Ours}          & RGB-D    & PSNR{[}dB{]}$\uparrow$   & \textbf{38.25} & \textbf{36.43}   & \textbf{38.11}   & \textbf{21.70}                         & \textbf{27.08}                         & \textbf{25.79}                          \\
              &          & SSIM$\uparrow$           & \textbf{0.97}  & \textbf{0.96}    & \textbf{0.96}    & \textbf{0.79}                          & \textbf{0.87}                          & \textbf{0.86}                           \\
              &          & LPIPS$\downarrow$        & \textbf{0.075} & \underline{0.081}   & \textbf{0.084}   & \textbf{0.252}                         & \textbf{0.113}                         & \textbf{0.169 }                         \\
              &          & ATE-MSE (cm)$\downarrow$ & \textbf{0.19}  & \underline{0.32}    & \textbf{0.40}    & \textbf{4.66}                          & \underline{0.42}                          & \textbf{0.31}        \\ \hline  
\end{tabular}
}
\caption{\textbf{Comparison with MonoGS~\cite{monogs}.} We conduct experiments both taking monocular RGB and RGB-D as input on Replica~\cite{replica} and TUM-RGBD~\cite{tum-rgbd} datasets, each consisting of 3 sequences. The best results are shown in \textbf{bold}, and the second best results are \underline{underlined}.}
\label{tab:tab_rgbd}
\end{table}

